Long-Term Photometric Consistent Novel View Synthesis with Diffusion Models

Novel view synthesis from a single input image is a challenging task, where the goal is to generate a new view of a scene from a desired camera pose that may be separated by a large motion. The highly uncertain nature of this synthesis task due to unobserved elements within the scene (i.e. occlusion) and outside the field-of-view makes the use of generative models appealing to capture the variety of possible outputs. In this paper, we propose a novel generative model capable of producing a sequence of photorealistic images consistent with a specified camera trajectory, and a single starting image. Our approach is centred on an autoregressive conditional diffusion-based model capable of interpolating visible scene elements, and extrapolating unobserved regions in a view, in a geometrically consistent manner. Conditioning is limited to an image capturing a single camera view and the (relative) pose of the new camera view. To measure the consistency over a sequence of generated views, we introduce a new metric, the thresholded symmetric epipolar distance (TSED), to measure the number of consistent frame pairs in a sequence. While previous methods have been shown to produce high quality images and consistent semantics across pairs of views, we show empirically with our metric that they are often inconsistent with the desired camera poses. In contrast, we demonstrate that our method produces both photorealistic and view-consistent imagery.

==> fig-tex/cons-gt-mp3d.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/mp3d/tsed-mp3d-spacing-1-long.pdf}
        % \vspace{-10pt}
    \caption{
    MP3D TSED on in-distribution trajectories.
    Consistency is measured as the average percent of consistent image pairs in the generated sequences. We set $T_\text{matches} = 10$.
    }
    \label{fig:cons-gt-mp3d}
        \vspace{-10pt}
\end{figure}

==> fig-tex/cons-gt.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/tsed-spacing-10-long.pdf}
        \vspace{-10pt}
    \caption{
    RealEstate10K TSED on in-distribution trajectories.
    Consistency is measured as the average percent of consistent image pairs in the generated sequences. We set $T_\text{matches} = 10$.
    }
    \label{fig:cons-gt}
        \vspace{-10pt}
\end{figure}

==> fig-tex/fid-novel-mp3d.tex <==
\begin{figure*}[t]
    \vspace{-10pt}
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mp3d/fids-mp3d-hop.pdf}
         \vspace{-20pt}
         % \caption{Hop}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mp3d/fids-mp3d-orbit.pdf}
         \vspace{-20pt}
         % \caption{Orbit}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mp3d/fids-mp3d-spin.pdf}
         \vspace{-20pt}
         % \caption{Spin}
     \end{subfigure}
     % \vspace{-5pt}
     \caption{
     MP3D FID scores on custom trajectories.
     Sequences are sampled using three novel trajectories designed to differ from the dominant modes in the dataset: Hop, Orbit, and Spin.
     }
     \label{fig:fid-novel-mp3d}
     \vspace{-5pt}
\end{figure*}

==> fig-tex/fid-novel.tex <==
\begin{figure*}
    \vspace{-10pt}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/fids-hop.pdf}
         \vspace{-20pt}
         % \caption{Hop}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/fids-orbit.pdf}
         \vspace{-20pt}
         % \caption{Orbit}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/fids-spin.pdf}
         \vspace{-20pt}
         % \caption{Spin}
     \end{subfigure}
     % \vspace{-5pt}
     \caption{
     RealEstate10K FID scores on custom trajectories.
     Sequences are sampled using three novel trajectories designed to differ from the dominant modes in the dataset: Hop, Orbit, and Spin.
     \textit{LookOut*} is a version of LookOut without error accumulation post-processing.
     }
     \label{fig:fid-novel}
     \vspace{-5pt}
\end{figure*}

==> fig-tex/tsed-novel-mp3d.tex <==
\begin{figure*}[t]
    \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mp3d/tsed-mp3d-hop.pdf}
         \vspace{-20pt}
         % \caption{Hop}
     \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mp3d/tsed-mp3d-orbit.pdf}
         \vspace{-20pt}
         % \caption{Orbit}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mp3d/tsed-mp3d-spin.pdf}
         \vspace{-20pt}
         % \caption{Spin}
     \end{subfigure}
     % \vspace{-5pt}
     \caption{
     MP3D TSED scores on custom trajectories.
     Plots for TSED over a range of $T_\text{error}$ values, with $T_\text{matches} = 10$, for our three custom trajectories: Hop, Orbit, and Spin. 
     }
     \label{fig:tsed-novel-mp3d}
\end{figure*}

==> fig-tex/tsed-novel.tex <==
\begin{figure*}
    \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/tsed-hop.pdf}
         \vspace{-20pt}
         % \caption{Hop}
     \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/tsed-orbit.pdf}
         \vspace{-20pt}
         % \caption{Orbit}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/tsed-spin.pdf}
         \vspace{-20pt}
         % \caption{Spin}
     \end{subfigure}
     \vspace{-5pt}
     \caption{
     RealEstate10K TSED scores on custom trajectories.
     We set $T_\text{matches} = 10$ while sweeping over a range of $T_\text{error}$ values, for our three custom trajectories: Hop, Orbit, and Spin.
     \textit{LookOut*} is a version of LookOut without error accumulation post-processing.}
     \label{fig:tsed-novel}
     % \vspace{-30pt}
\end{figure*}

==> fig-tex/tsed-sensitivity.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/sensitivity/gt_fb.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/sensitivity/gt_lr.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/sensitivity/gt_azi.pdf}
    \end{subfigure}
    \vspace{-8pt}
    \caption{
    TSED sensitivity analysis for image pairs with different dominant camera motions using $T_\text{error}=2$.
    TSED scores are plotted for perturbations to the 2D correspondence locations with constant magnitude along horizontal and vertical directions.
    Camera motion determines the orientations of the epipolar lines, which can make the metric insensitive in some cases when many epipolar lines share the same orientation.
    }
    \label{fig:tsed-sensitivity}
    \vspace{-10pt}
\end{figure*}

==> table-tex/FID-gt-mp3d.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    %\resizebox{\linewidth}{!}{
    \begin{tabular}{c|cc}
        Method & Short-term FID $\downarrow$ & Long-term FID $\downarrow$ \\
        \hline
        LookOut \cite{ren2022look}  & 80.97 & 132.36 \\
        Ours                        & \textbf{73.16} & \textbf{100.99} \\
    \end{tabular}
    %}
    \caption{
    MP3D FIDs with in-distribution trajectories.
    FID scores between generated images at short and long term generations, and a fixed set of randomly selected images from the MP3D test set.
    Generated images are along in-distribution trajectories.
    }
    \vspace{-1em}
    \label{tab:FID-gt-mp3d}
\end{table}

==> table-tex/FID-gt.tex <==
\begin{table}
    \centering
    \footnotesize
    %\resizebox{\linewidth}{!}{
    \begin{tabular}{c|cc}
        Method & Short-term FID $\downarrow$ & Long-term FID $\downarrow$ \\
        \hline
        GeoGPT \cite{rombach2021geometry}  & \textbf{26.72} & \textbf{41.87} \\
        LookOut-noerror \cite{ren2022look} & 30.38 & 72.01 \\
        LookOut \cite{ren2022look} & 28.86 & 58.12 \\
        Ours    & 26.76 & 41.95 \\
    \end{tabular}
    %}
    \caption{
    RealEstate10K FIDs with in-distribution trajectories.
    FID scores between generated images at short and long term generations, and a fixed set of randomly selected images from the test set.
    Generated images are along in-distribution trajectories.}
       \vspace{-10pt}
    \label{tab:FID-gt}
\end{table}

==> table-tex/recon-gt-mp3d.tex <==
\begin{table}[t]
    \footnotesize
    \centering
    \begin{tabular}{c|cc|cc}
        \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Short} & \multicolumn{2}{c}{Long} \\
             & LPIPS $\downarrow$ & PSNR $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ \\
        \hline
        LookOut \cite{ren2022look} & 0.604 & 12.76 & 0.739 & 10.60 \\ 
        Ours                       & \textbf{0.504} & \textbf{14.83} & \textbf{0.674} & \textbf{13.00}
    \end{tabular}
    \caption{
    MP3D reconstruction metrics with in-distribution trajectories.}
    \label{tab:full-matterport-recon}
    \vspace{-2em}
\end{table}

==> table-tex/recon-gt.tex <==
\begin{table}
    \footnotesize
    \centering
    %\resizebox{\linewidth}{!}{
    \begin{tabular}{c|cc|cc}
        \multirow{2}{*}{Method}  & \multicolumn{2}{c|}{Short-term} & \multicolumn{2}{c}{Long-term} \\
         & LPIPS $\downarrow$ & PSNR $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ \\
        \hline
        GeoGPT \cite{rombach2021geometry}  & 0.444 & 13.35 & 0.674 & 9.54 \\
        LookOut-noerror \cite{ren2022look} & 0.390 & 14.19 & 0.688 & 9.65 \\
        LookOut \cite{ren2022look} & 0.378 & 14.43 & 0.658 & 10.51 \\
        Ours    & \textbf{0.333} & \textbf{15.51} & \textbf{0.588} & \textbf{11.54} \\
    \end{tabular}
    %}
    \caption{
    Realestate10K reconstruction metrics with in-distribution trajectories.
    LookOut-noerror refers to the LookOut method without the final error accumulation training step.}
       \vspace{-10pt}
    \label{tab:recon-gt}
\end{table}
